Smoothing Method for Approximate Extensive-Form Perfect Equilibrium

Nash equilibrium is a popular solution concept for solving imperfect-information games in practice. However, it has a major drawback: it does not preclude suboptimal play in branches of the game tree that are not reached in equilibrium. Equilibrium refinements can mend this issue, but have experienced little practical adoption. This is largely due to a lack of scalable algorithms. Sparse iterative methods, in particular first-order methods, are known to be among the most effective algorithms for computing Nash equilibria in large-scale two-player zero-sum extensive-form games. In this paper, we provide, to our knowledge, the first extension of these methods to equilibrium refinements. We develop a smoothing approach for behavioral perturbations of the convex polytope that encompasses the strategy spaces of players in an extensive-form game. This enables one to compute an approximate variant of extensive-form perfect equilibria. Experiments show that our smoothing approach leads to solutions with dramatically stronger strategies at information sets that are reached with low probability in approximate Nash equilibria, while retaining the overall convergence rate associated with fast algorithms for Nash equilibrium. This has benefits both in approximate equilibrium finding (such approximation is necessary in practice in large games) where some probabilities are low while possibly heading toward zero in the limit, and exact equilibrium computation where the low probabilities are actually zero.

==> approximate_efpe.tex <==
\section{Perturbed Sequence-Form Polytopes}
\begin{definition}
  The perturbed sequence-form polytope {\Xeps} is the sequence-form polytope $\cX$ with the additional constraint
\[
  x_i \geq \e^{d_j}, \forall j\in S_\cX, i \in \bbI_j.
\]
{\Yeps} is the analogous perturbation of $\cY$.
\end{definition}

\section{Approximate Sequential Equilibria}
\todo{Change definition to be local to each infoset?}
\begin{definition}[$\epsilon$-$\delta$-sequential equilibrium]
  An {\edqpe} is a strategy pair 
  $x\in \Xeps, y\in \Yeps$ such that
  \begin{align}
    \label{eq:edqpe}
    f^\e(x) - \phi^\e(y) \le \delta
  \end{align}
\end{definition}
\begin{observation}
  As $\e,\delta \rightarrow 0$, an {\edqpe} converges to a quasi-perfect
  equilibrium.
\end{observation}

\todo{Fix the theorem below}
\begin{proposition}
  An {\edqpe} constitutes a $( |Z|\e^d \|A\| + \delta )$-Nash equilibrium.
\end{proposition}
\begin{proof}
  We show the result for best responding to $y$, with the analogous argument
  holding for $x$. Since (\ref{eq:edqpe}) holds we have that any best response
  $x^*$ within $\Xeps$ leads to at most $\delta$ regret. Now, we further have
  that for any $\hat{x}\in \Xeps$
\end{proof}

==> sequence_form.tex <==
\subsection{Sequence Form}
It is well-known that the strategy spaces of an extensive-form game can be transformed into convex polytopes that allow a bilinear saddle-point formulation of the Nash equilibrium problem as follows~\cite{Romanovskii62:Reduction,Stengel96:Efficient,Koller96:Efficient}
\begin{equation}
  \label{eq:sequence_form_objective} \min_{x \in \cX} \max_{y \in \cY} \langle
x, Ay \rangle = \max_{y \in \cY} \min_{x \in \cX} \langle x,Ay \rangle .
\end{equation}
Our approach for computing Nash-equilibrium refinements will be based on constructing a perturbed variant of $\cX$ and $\cY$.
